A Fundamental Accuracy--Robustness Trade-off in Regression and Classification

We derive a fundamental trade-off between standard and adversarial risk in a rather general situation that formalizes the following simple intuition: "If no (nearly) optimal predictor is smooth, adversarial robustness comes at the cost of accuracy." As a concrete example, we evaluate the derived trade-off in regression with polynomial ridge functions under mild regularity conditions. Generalizing our analysis of this example, we formulate a necessary condition under which adversarial robustness can be achieved without significant degradation of the accuracy. This necessary condition is expressed in terms of a quantity that resembles the Poincar\'{e} constant of the data distribution.

==> preamble.tex <==
% \PassOptionsToPackage{natbib=true}{biblatex}
\usepackage[T1]{fontenc}
\usepackage[latin9]{inputenc}
\usepackage{amsmath, amsthm}
\usepackage{enumitem}
\usepackage{csquotes}

\makeatletter
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Textclass specific LaTeX commands.
\theoremstyle{plain}
\newtheorem{thm}{\protect\theoremname}
\newtheorem{cor}{\protect\corollaryname}
\newtheorem{lem}{\protect\lemmaname}
\newtheorem{prop}{\protect\propositionname}
\theoremstyle{definition}
\newtheorem{defn}{\protect\definitionname}
\newtheorem{exmp}{\protect\examplename}
\newtheorem*{exmp*}{\protect\examplename}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% User specified LaTeX commands.
\ifcsname noxcolor\endcsname
	\usepackage[serif,no-xcolor]{macros4tex}
\else
	\usepackage[serif]{macros4tex}
\fi

\usepackage[unicode=true,pdfusetitle,
	bookmarks=true,bookmarksnumbered=false,bookmarksopen=false,
	breaklinks=false,pdfborder={0 0 0},pdfborderstyle={},backref=false,colorlinks=true]
{hyperref}
\ifcsname noxcolor\endcsname
\else
	\hypersetup{
		urlcolor = URLColor,
		citecolor = CiteColor,
		linkcolor = LinkColor}
\fi

\usepackage[capitalise, noabbrev, nameinlink]{cleveref}
\crefname{thm}{Theorem}{Theorems}
\crefname{lem}{Lemma}{Lemmas}
\crefname{cor}{Corollary}{Corollary}
\crefname{prop}{Proposition}{Propositions}
\crefname{defn}{Definition}{Definitions}
\crefname{exmp}{Example}{Examples}
\crefname{problem}{Problem}{Problems}
\crefname{figure}{Figure}{Figures}
\crefname{table}{Table}{Tables}
\crefformat{equation}{#2#1#3}


\AtBeginDocument{
	\ifcsname nobiblatex\endcsname
	\else
		%\DeclareFieldFormat{labelalpha}{\thefield{entrykey}}
		%\DeclareFieldFormat{extraalpha}{}
		\DeclareFieldFormat{titlecase:title}{\MakeSentenceCase*{#1}}
		\DeclareFieldFormat{titlecase:maintitle}{#1}
		\renewbibmacro{in:}{}
		\renewcommand*{\volnumdelim}{\addcolon\space}
	\fi
	\renewcommand*{\ref}[1]{\cref{#1}}
}

% \usepackage{geometry}
% \geometry{verbose,tmargin=1in,bmargin=1in,lmargin=1in,rmargin=1in}

% \usepackage{refcheck}
% \newcommand{\refcheckize}[1]{%
%   \expandafter\let\csname @@\string#1\endcsname#1%
%   \expandafter\DeclareRobustCommand\csname relax\string#1\endcsname[1]{%
%     \csname @@\string#1\endcsname{##1}\wrtusdrf{##1}}%
%   \expandafter\let\expandafter#1\csname relax\string#1\endcsname
% }
% \refcheckize{\cref}
% \refcheckize{\Cref}
\makeatother
%%%

%%% Now we add the reference commands we want refcheck to be aware of
% \refcheckize{\cref}
% \refcheckize{\Cref}

\usepackage[english]{babel}

\ifcsname nobiblatex\endcsname
\else
	\ifcsname stylebib\endcsname%
	\else%
		\def\stylebib{ext-numeric}
	\fi%

	% \def\stylebib{ext-numeric}
	\usepackage[style=\stylebib, %ext-alphabetic, 
		backend=biber, natbib=true, backref=true, giveninits=true, useprefix = true, sorting=nyt, url=false, isbn=false, eprint=true, doi=false, maxalphanames=4, minalphanames=4, minbibnames=6, maxbibnames=99]{biblatex}

	\AtEveryBibitem{
		\ifentrytype{book}{}{% Remove publisher and editor except for books
			\clearlist{publisher}
			\clearname{editor}
		}
	}
	\DeclareFieldFormat{titlecase:title}{\MakeSentenceCase*{#1}}
	% \DeclareFieldFormat{titlecase:maintitle}{#1}
	\renewbibmacro{in:}{}
\fi

\providecommand{\lemmaname}{Lemma}
\providecommand{\propositionname}{Proposition}
\providecommand{\corollaryname}{Corollary}
\providecommand{\theoremname}{Theorem}
\providecommand{\definitionname}{Definition}
\providecommand{\examplename}{Example}

